Learning Anatomically Consistent Embedding for Chest Radiography

Self-supervised learning (SSL) approaches have recently shown substantial success in learning visual representations from unannotated images. Compared with photographic images, medical images acquired with the same imaging protocol exhibit high consistency in anatomy. To exploit this anatomical consistency, this paper introduces a novel SSL approach, called PEAC (patch embedding of anatomical consistency), for medical image analysis. Specifically, in this paper, we propose to learn global and local consistencies via stable grid-based matching, transfer pre-trained PEAC models to diverse downstream tasks, and extensively demonstrate that (1) PEAC achieves significantly better performance than the existing state-of-the-art fully/self-supervised methods, and (2) PEAC captures the anatomical structure consistency across views of the same patient and across patients of different genders, weights, and healthy statuses, which enhances the interpretability of our method for medical image analysis.

==> jl_defs_20230719_1618.tex <==
%%=================================================================================================%%
%% Use the conditions to turn off colors and comments -- Do NOT edit this file after the conditions%%
%%=================================================================================================%%
\newif\ifSubmitting
  \Submittingtrue 
  %\Submittingfalse

\newif\ifPreparing
 %\Preparingtrue 
 \Preparingfalse

\newif\ifIPreparing
  %\IPreparingtrue 
  \IPreparingfalse

\newif\ifIIPreparing
  %\IIPreparingtrue 
  \IIPreparingfalse

\newif\ifIIIPreparing
  %\IIIPreparingtrue 
  \IIIPreparingfalse
  
\newif\ifIVPreparing
  \IVPreparingtrue 
  %\IVPreparingfalse
  
\newif\ifVPreparing
  \VPreparingtrue 
  %\VPreparingfalse

\input{jl_defs_body_20230615_1351}
%\renewenvironment{jlblue}{\color{orange}}{}

==> jp_defs.tex <==
\usepackage{ulem,lipsum}
\newcommand\jpxoutpars[1]{\let\helpcmd\xout\parhelp#1\par\relax\relax}
\newcommand\jpsoutpars[1]{\let\helpcmd\sout\parhelp#1\par\relax\relax}
\long\def\parhelp#1\par#2\relax{%
  \helpcmd{#1}\ifx\relax#2\else\par\parhelp#2\relax\fi%
}


%%=================================================================================================%%
%% Use the conditions to turn off colors and comments -- Do NOT edit this file after the conditions%%
%%=================================================================================================%%
\newif\ifSubmitting
  %\Submittingtrue 
  \Submittingfalse

\newif\ifPreparing
  % \Preparingtrue 
  \Preparingfalse

\newif\ifSecondPreparing
  %\SecondPreparingtrue 
  \SecondPreparingfalse

\newif\ifThirdPreparing
  \ThirdPreparingtrue 
  %\ThirdPreparingfalse

%%========================================================================================%%
%% Use the conditions to turn off colors and comments -- Do NOT edit the rest of this file%%
%%========================================================================================%%
\ifSubmitting 
    \Preparingfalse
    \SecondPreparingfalse
    \ThirdPreparingfalse
\fi
\usepackage{soul}  

\newcommand{\jladvancedreplace}[2]{{\jlgray\st{#1}}{\jlblue #2}}

\ifPreparing
%% Colors
    \newenvironment{jlblack}{\color{black}}{}
    \newenvironment{jlblue}{\color{blue}}{}
    \newenvironment{jlred}{\color{red}}{}
    \newenvironment{jlmagenta}{\color{magenta}}{}
    \newenvironment{jlorange}{\color{orange}}{}
    \newenvironment{jltan}{\color{tan}}{}
    \newenvironment{jlgray}{\color{gray}}{}
    \newenvironment{jllightgray}{\color{lightgray}}{}
%% Commands 
    \newcommand{\jldelete}[1]{{\jlred\st{#1}}}
\else
%% turn off all colors
    \newenvironment{jlblack}{\color{black}}{}
    \newenvironment{jlblue}{}{}
    \newenvironment{jlred}{}{}
    \newenvironment{jlmagenta}{}{}
    \newenvironment{jlorange}{}{}
    \newenvironment{jltan}{}{}
    \newenvironment{jlgray}{}{}
    \newenvironment{jllightgray}{}{}
\fi
%% Commands
    \newcommand{\jpreplace}[2]{{\jlorange #2}}
    \newcommand{\jpinsert}[1]{{\jlblue #1}}

    \newcommand{\jpnote}[2]{{\jlmagenta [#1]}{{\jlgray #2}}}
    \newcommand{\jpdelete}[1]{} 
    \newenvironment{dmcolor}{\color{black}}{}
    \newcommand{\dmreplace}[2]{{\dmcolor #2}} 
    \newcommand{\dmnote}[2]{{\dmcolor [#1]}{{\jlgray #2}}}
    \newcommand{\dmcleandelete}[1]{}
%%
